Context-Aided Variable Elimination for Requirement Engineering

Deriving system-level specifications from component specifications usually involves the elimination of variables that are not part of the interface of the top-level system. This paper presents algorithms for eliminating variables from formulas by computing refinements or relaxations of these formulas in a context. We discuss a connection between this problem and optimization and give efficient algorithms to compute refinements and relaxations of linear inequality constraints.

==> appendices/proofs.tex <==














  






==> sections/partialorders.tex <==


\newcommand{\fcal}[0]{\mathcal{F}}
\newcommand{\rcal}[0]{\mathcal{R}}
\newcommand{\mcal}[0]{\mathcal{M}}

\newcommand{\ffcal}[0]{\mathcal{F}^\mcal}
\newcommand{\rrcal}[0]{\mathcal{R}^\mcal}
\newcommand{\ddcal}[0]{\mathcal{D}_\mcal}


In this section, we consider the computation of antecedents and consequents of atomic formulas from a first-order theory in a structure endowed with a partial order. We establish a link between this problem and optimization. Our attention will be on atomic formulas of the form $f(x, g(y)) \le K$, where $y$ is an array of irrelevant variables and $f$ is monotonic in the second argument. In other words, we assume that the irrelevant variables can be separated from the rest of the variables in the formula. We use a context $\Gamma$ to bound $g(y)$ using an expression that does not depend on $y$. This allows us to eliminate irrelevant variables from the original formula. We show that this framework supports formula refinement/relaxation for propositional logic and linear inequalities.

\medskip

Our description of formal languages borrows notation from \cite{pinchinat2022logique}. 
Let $(\fcal, \rcal)$ be the signature of the first order language $L$ and let $V$ be a set of variables.
That is, let $\fcal$ and $\rcal$ be sets of function and relation symbols of various arities.
Let $\mcal = (\ddcal, \ffcal, \rrcal)$ be a structure in which we interpret $L$. Here $\ddcal$ is a set called the domain. For each function symbol $f\in \fcal$ of arity $n$, there is $f^\mcal \in \ffcal$ such that $f^\mcal \colon \ddcal^n \to \ddcal$; and for each $m$-ary relation symbol $R\in \rcal$, we have $R^\mcal \in \rrcal$ such that $R^\mcal \subseteq \ddcal^m$.

We will assume that $\ddcal$ is a bounded, complete partial order and that $\rcal$ contains a binary relation, denoted $\le$, whose interpretation $\le_\mcal$ in $\mcal$ is the partial order relation of $\ddcal$.

Let $X = \{x_i\}_{i = 1}^m \subseteq V$ and $Y = \{y_i\}_{i = 1}^n \subseteq V$ be disjoint sets of variables, where the elements of $Y$ will be called \emph{irrelevant variables}.
Suppose $K \in \fcal$ is a $0$-ary (a constant) function symbol, $f$ is an $(m+1)$-ary term generated by $\fcal$ and $X \setunion Y$, and $g$ is an $n$-ary term generated by $\fcal$ and $Y$. Moreover, suppose that the function $f^\mcal$ is monotonic in its last argument. This is the problem we want to solve:

\mybox{Given an atomic formula $\phi$ of the form
\begin{equation}\label{monhlk}
\phi\colon \quad f(x_1, \ldots, x_m, g(y_1, \ldots, y_n)) \le K,
\end{equation}
a set of formulas $\Gamma$, and a structure $\mcal$,
synthesize an antecedent or consequent of the atomic formula $\phi$ in the context $\Gamma$
when the formulas are interpreted in $\mcal$. The resulting formulas cannot contain irrelevant variables.
}

We assume that the context $\Gamma$ contains, in addition to irrelevant variables and $X$ variables, a set of variables $Z = \{z_i\}_{i = 1}^o$ disjoint from $X$ and $Y$. From now on, we will keep the following notation: $m$ denotes the number of variables that do not need to be eliminated from $\phi$, $n$ the number of irrelevant variables in $\phi$, $o$ the number of $Z$ variables in $\Gamma$, and $N$ the number of formulas in $\Gamma$.

\medskip
\newcommand\mydots{\hbox to 0.9em{.\hss.\hss.}}

We define functions $g_+^\mcal, g_-^\mcal\colon \ddcal^{m+o} \to \ddcal$ as follows:
{\small
\begin{align}\label{lqdhllq}
g_+^\mcal(a_1, \ldots, a_m,c_1, \ldots, c_o) =
\begin{cases}
\begin{aligned}[t]
%& \bottom & &, \text{if } \\
& \underset{b_1, \ldots, b_n \in \ddcal}{\text{maximize}}
& & g^\mcal(b_1, \ldots, b_n) \\
& \text{subject to}
& & \mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models \Gamma
\end{aligned}
\end{cases}
\end{align}
}
and
{\small
\begin{align}
\label{kwbgf}
g_-^\mcal(a_1, \ldots, a_m,c_1, \ldots, c_o) =
\begin{cases}
\begin{aligned}[t]
%& \bottom & &, \text{if } \\
& \underset{b_1, \ldots, b_n \in \ddcal}{\text{minimize}}
& & g^\mcal(b_1, \ldots, b_n) \\
& \text{subject to}
& & \mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models \Gamma,
\end{aligned}
\end{cases}
\end{align}}
where the notation
$\mcal, [x \coloneqq a, y \coloneqq b, z \coloneqq c]$ means that the formula is satisfied in the structure $\mcal$ after substituting the variables $x_i$ by $a_i$, $y_i$ by $b_i$, and $z_i$ by $c_i$. $g_+^\mcal$ and $g_-^\mcal$ are well defined because $\ddcal$ is complete and bounded.

We assume that the term algebra generated by $\fcal$ and $X\setunion Z$ contains $(m+o)$-ary terms $g_+$ and $g_-$ whose interpretations in $\mcal$ are $g_+^\mcal$ and $g_-^\mcal$, respectively. We have the following result:

\begin{theorem}\label{knhlxh}
Let $\phi'$ and $\phi''$ be
\begin{equation}\label{lniyxuy}
\phi'\colon \quad f(x_1, \ldots, x_m, g_+(x_1, \ldots, x_m, z_1, \ldots, z_o)) \le K
\end{equation}
and
\begin{equation}\label{hnqoif}
\phi''\colon \quad f(x_1, \ldots, x_m, g_-(x_1, \ldots, x_m, z_1, \ldots, z_o)) \le K.
\end{equation}
These formulas satisfy
$\mcal \models (\Gamma \land \phi')\Rightarrow \phi$
and
$\mcal \models (\Gamma \land \phi)\Rightarrow \phi''$.
\end{theorem}
\begin{proof}
Let $a_i, b_j, c_k \in \ddcal$ for $i \le m$, $j \le n$, and $k \le o$.
First we will show that
\begin{equation}\label{nqklgk}
\mcal \models \Gamma \Rightarrow (g(y_1, \ldots y_n) \le g_+(x_1, \ldots, x_m, z_1, \ldots z_o)).
\end{equation}
If $\mcal, [x \coloneqq a, y \coloneqq b, z\coloneqq c] \not \models \Gamma$, the result holds vacuously. 
If $\mcal, [x \coloneqq a, y \coloneqq b, z\coloneqq c] \models \Gamma$, then from \eqref{lqdhllq} we have
$$g^\mcal(b_1, \ldots, b_n) \le_\mcal g_+^\mcal (a_1, \ldots, a_m, c_1, \ldots, c_o),$$
showing that \eqref{nqklgk} holds.
\medskip

Suppose $\mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models (\Gamma \land \phi')$. We have from \eqref{nqklgk}
$$\mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models (g(y_1, \ldots y_n) \le g_+(x_1, \ldots, x_m, z_1, \ldots z_o)).$$
It follows that
$$
\mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models \phi' \land (g(y_1, \ldots y_n) \le g_+(x_1, \ldots, x_m, z_1, \ldots z_o)),
$$
which means that
\begin{align*}
&(f^\mcal(a_1, \ldots, a_m, g^\mcal_+(a_1, \ldots, a_m, c_1, \ldots, c_o)) \le_\mcal K^\mcal) \land \\
&(g^\mcal(b_1, \ldots b_n) \le_\mcal g_+^\mcal(a_1, \ldots, a_m, c_1, \ldots c_o)).
\end{align*}
Since $f^\mcal$ is monotonic in the last argument, we obtain
$$
f^\mcal(a_1, \ldots, a_m, g^\mcal(b_1, \ldots b_n)) \le_\mcal K^\mcal.
$$
Thus, $\mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models \phi$, proving the first part of the theorem.

We will prove that
\begin{equation}\label{bfnh}
    \mcal \models \Gamma \Rightarrow (g_-(x_1, \ldots, x_m, z_1, \ldots z_o) \le g(y_1, \ldots y_n)).
\end{equation}
Suppose $\mcal, [x \coloneqq a, y \coloneqq b, z\coloneqq c] \models \Gamma$, then from \eqref{kwbgf} we have
$$g_-^\mcal (a_1, \ldots, a_m, c_1, \ldots, c_o) \le_\mcal g^\mcal(b_1, \ldots, b_n),$$ showing that \eqref{bfnh} holds.
\medskip

Suppose $\mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models (\Gamma \land \phi)$. We have from \eqref{bfnh}
$$\mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models (g_-(x_1, \ldots, x_m, z_1, \ldots z_o) \le g(y_1, \ldots y_n)).$$
It follows that
$$
\mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models \phi \land (g_-(x_1, \ldots, x_m, z_1, \ldots z_o) \le g(y_1, \ldots y_n)),
$$
which means that
\begin{align*}
&(f^\mcal(a_1, \ldots, a_m, g^\mcal(b_1, \ldots b_n)) \le_\mcal K^\mcal) \land \\
&(g_-^\mcal(a_1, \ldots, a_m, c_1, \ldots c_o) \le_\mcal g^\mcal(b_1, \ldots b_n)).
\end{align*}
Since $f^\mcal$ is monotonic in the last argument, we conclude that
$$
f^\mcal(a_1, \ldots, a_m, g^\mcal_-(a_1, \ldots, a_m, c_1, \ldots, c_o)) \le_\mcal K^\mcal.
$$
Thus, $\mcal, [x\coloneqq a, y \coloneqq b, z \coloneqq c] \models \phi''$, proving the second part.
\end{proof}

Theorem \ref{knhlxh} 
gives us antecedents and consequents of atomic formulas $\phi$ of the form \eqref{monhlk} such that the result lacks irrelevant variables.

\begin{example}
Suppose $(\fcal, \rcal)$ is the signature of a propositional language and $\rcal$ only contains a binary relation $\le$.
We will interpret this language in the model $\mcal$ with domain $\{0,1\}$, where we will assume that $0 \le_\mcal 1$.
Suppose we want to compute antecedents and consequents of the formula
$$\phi\colon (p \land q) \lor r,$$
in the context $\Gamma\colon s \Rightarrow q$, where $q$ is an irrelevant variable. We can apply Theorem \ref{knhlxh} as follows:
We observe that $\Rightarrow$ and $\le$ have the same semantics in $\mcal$. Thus, we can write $\phi$ as $\phi\colon (\neg p \lor \neg q) \le r$.
Let $g(q) = \neg q$ and $f(p, x) = \neg p \lor x$. Then $f^\mcal$ is monotonic in its last argument. To apply Theorem \ref{knhlxh}, we compute $g_+^\mcal$:
\begin{align*}
    g_+^\mcal(a,c) =
    \begin{cases}
    \begin{aligned}[t]
    %& \bottom & &, \text{if } \\
    & \underset{b \in \{0,1\}}{\text{maximize}}
    & & \neg q \\
    & \text{subject to}
    & & \mcal, [p\coloneqq a, q \coloneqq b, s\coloneqq c] \models s \le q
    \end{aligned}
    \end{cases}
=
\neg c.
\end{align*}
Thus, $g_+(p,s) = \neg s$. By Theorem \ref{knhlxh}, we conclude that $f(p, g_+(p,s)) \le r$ is an antecedent of $\phi$ in the given context, i.e., we compute
$$
\neg p \lor \neg s \le r,
$$
which is equivalent to
$(p \land s) \lor r$.
\qeda
\end{example}



==> sections/previouswork.tex <==

%Deduction and abduction are formalized in philosophy. Aristotle defines deduction as ``speech (logos) in which, certain things having been supposed, something different from those supposed results of necessity because of their being so'' \cite{sep-aristotle-logic}. Much more recently, Peirce defines abduction as ``the process of forming explanatory hypotheses'' %It is the only logical operation which introduces any new idea''
%\cite{sep-abduction}. For our purposes, these two mechanisms of reasoning will have the following meaning. Let $\phi$ be a formula in a theory and let $\Gamma$ be a set of formulas serving as context. The deduction and abduction problems are
%\begin{align*}
%    &\Gamma \land \phi \models \text{ ? } \text{ (deduction)}
%    && \text{and}
%    &&&\Gamma \land \text{ ? } \models \phi \text{ (abduction),}
%\end{align*}
%i.e., in deduction we look for a consequent; in abduction we look for an antecedent.

****** Literature summary incomplete.

Automated deduction is a vast research subject, as witnessed by N. Shankar's excellent overview \cite{10.1145/1592434.1592437}.


Eiter and Gottlob \cite{10.1145/200836.200838} provide an overview of abduction in Computer Science


Dillig and her collaborators make use of abduction to aid the classification of errors flagged by program verification tools \cite{DilligErrorDiagnosis}. Their method uses abductive reasoning to compute queries to be presented to the user in order for the verification program to obtain the missing information required to either confirm or reject the error. In \cite{dilligIndInvariants}, they use abduction to compute inductive loop invariants. They adopt Presburger arithmetic as the constraint language, and their implementation of abduction is based on quantifier elimination. I. and T. Dillig provide a tool named Explain \cite{isilExplain} for abducing terms expressed in Presburger arithmetic. To ensure the simplify of the computed abductions, Explain generates terms having as few variables as possible; moreover, the generated abduced terms are the weakest possible (but not necessarily unique) among the allowed solutions.


Echenim et al. \cite{10.1007/978-3-030-29007-8} 


Calcano et al. \cite{10.1145/1480881.1480917}

Ignatiev et al. \cite{10.3233/978-1-61499-672-9-1327}


Piscak et a.. \cite{10.1007/978-3-642-39799-8-54}

Cousot et al.\cite{10.1007/978-3-642-35873-9-10} 

Seghir et al. \cite{10.1007/978-3-642-37036-6-25}

Reynolds et al. \cite{10.1007/978-3-030-51074-9-9}

Gorogiannis et al. \cite{10.1007/978-3-642-23702-7-7}


Let et al. \cite{10.1007/978-3-319-08867-9-4}


